GPS-SSL: Guided Positive Sampling to Inject Prior Into Self-Supervised Learning

We propose Guided Positive Sampling Self-Supervised Learning (GPS-SSL), a general method to inject a priori knowledge into Self-Supervised Learning (SSL) positive samples selection. Current SSL methods leverage Data-Augmentations (DA) for generating positive samples and incorporate prior knowledge - an incorrect, or too weak DA will drastically reduce the quality of the learned representation. GPS-SSL proposes instead to design a metric space where Euclidean distances become a meaningful proxy for semantic relationship. In that space, it is now possible to generate positive samples from nearest neighbor sampling. Any prior knowledge can now be embedded into that metric space independently from the employed DA. From its simplicity, GPS-SSL is applicable to any SSL method, e.g. SimCLR or BYOL. A key benefit of GPS-SSL is in reducing the pressure in tailoring strong DAs. For example GPS-SSL reaches 85.58% on Cifar10 with weak DA while the baseline only reaches 37.51%. We therefore move a step forward towards the goal of making SSL less reliant on DA. We also show that even when using strong DAs, GPS-SSL outperforms the baselines on under-studied domains. We evaluate GPS-SSL along with multiple baseline SSL methods on numerous downstream datasets from different domains when the models use strong or minimal data augmentations. We hope that GPS-SSL will open new avenues in studying how to inject a priori knowledge into SSL in a principled manner.

==> 0000authors.tex <==

% List of affiliations: The first argument should be a (short)
% identifier you will use later to specify author affiliations
% Academic affiliations should list Department, University, City, Region, Country
% Industry affiliations should list Company, City, Region, Country

% You can specify symbols, otherwise they are numbered in order.
% Ideally, you should not use this facility. Affiliations will be numbered
% in order of appearance and this is the preferred way.


% \icmlsetsymbol{equal}{*}

\author{Antiquus S.~Hippocampus, Natalia Cerebro \& Amelie P. Amygdale \thanks{ Use footnote for providing further information
about author (webpage, alternative address)---\emph{not} for acknowledging
funding agencies.  Funding acknowledgements go at the end of the paper.} \\
Department of Computer Science\\
Cranberry-Lemon University\\
Pittsburgh, PA 15213, USA \\
\texttt{\{hippo,brain,jen\}@cs.cranberry-lemon.edu} \\
\And
Ji Q. Ren \& Yevgeny LeNet \\
Department of Computational Neuroscience \\
University of the Witwatersrand \\
Joburg, South Africa \\
\texttt{\{robot,net\}@wits.ac.za} \\
\AND
Coauthor \\
Affiliation \\
Address \\
\texttt{email}
}



% \begin{icmlauthorlist}
% % \icmlauthor{Aarash Feizi}{equal, mcgill, mila}
% \icmlauthor{Aarash Feizi}{mcgill,mila}
% \icmlauthor{Arantxa	Casanova}{pt,mila}
% \icmlauthor{Adriana	Romero-Soriano}{mcgill,mila}
% \icmlauthor{Reihaneh Rabbany}{mcgill,mila}

% %\icmlauthor{}{sch}
% %\icmlauthor{}{sch}
% \end{icmlauthorlist}

% \icmlaffiliation{mcgill}{McGill University, Montr\'eal, Canada}

% \icmlaffiliation{mila}{Mila Institute, Montr\'eal, Canada}

% \icmlaffiliation{pt}{\'Ecole Polytechnique de Montr\'eal, Montr\'eal, Canada}

% \icmlcorrespondingauthor{Aarash Feizi}{aarash.feizi@mila.quebec}
% % \icmlcorrespondingauthor{Firstname2 Lastname2}{first2.last2@www.uk}




% \author{Aarash Feizi}
% % \authornote{Both authors contributed equally to this research.}
% \email{aarash.feizi@mail.mcgill.ca}
% \affiliation{%
%   \institution{CSC McGill}
%   \institution{Mila, Quebec AI Institute}
% }

% \author{Arantxa Casanova}
% \email{arantxa.casanova-paga@polymtl.ca}
% \affiliation{%
%   \institution{\'Ecole Polytechnique de Montr\'eal}
%   \institution{Mila, Quebec AI Institute}}


% \author{Adriana Romero-Soriano}
% \email{adriana.romerosoriano@mcgill.ca}
% \affiliation{%
%   \institution{SCS McGill}
%   \institution{Mila, Quebec AI Institute}}


% \author{Reihaneh Rabbany}
% \email{rrabba@cs.mcgill.ca}
% \affiliation{%
%   \institution{SCS McGill}
%   \institution{Mila, Quebec AI Institute}
% }



% \author{Ben Trovato}
% \authornote{Both authors contributed equally to this research.}
% \email{trovato@corporation.com}
% \orcid{1234-5678-9012}
% \author{G.K.M. Tobin}
% \authornotemark[1]
% \email{webmaster@marysville-ohio.com}
% \affiliation{%
%   \institution{Institute for Clarity in Documentation}
%   \streetaddress{P.O. Box 1212}
%   \city{Dublin}
%   \state{Ohio}
%   \country{USA}
%   \postcode{43017-6221}
% }

% \author{Lars Th{\o}rv{\"a}ld}
% \affiliation{%
%   \institution{The Th{\o}rv{\"a}ld Group}
%   \streetaddress{1 Th{\o}rv{\"a}ld Circle}
%   \city{Hekla}
%   \country{Iceland}}
% \email{larst@affiliation.org}

% \author{Valerie B\'eranger}
% \affiliation{%
%   \institution{Inria Paris-Rocquencourt}
%   \city{Rocquencourt}
%   \country{France}
% }

% \author{Aparna Patel}+
% \affiliation{%
%  \institution{Rajiv Gandhi University}
%  \streetaddress{Rono-Hills}
%  \city{Doimukh}
%  \state{Arunachal Pradesh}
%  \country{India}}

% \author{Huifen Chan}
% \affiliation{%
%   \institution{Tsinghua University}
%   \streetaddress{30 Shuangqing Rd}
%   \city{Haidian Qu}
%   \state{Beijing Shi}
%   \country{China}}

% \author{Charles Palmer}
% \affiliation{%
%   \institution{Palmer Research Laboratories}
%   \streetaddress{8600 Datapoint Drive}
%   \city{San Antonio}
%   \state{Texas}
%   \country{USA}
%   \postcode{78229}}
% \email{cpalmer@prl.com}

% \author{John Smith}
% \affiliation{%
%   \institution{The Th{\o}rv{\"a}ld Group}
%   \streetaddress{1 Th{\o}rv{\"a}ld Circle}
%   \city{Hekla}
%   \country{Iceland}}
% \email{jsmith@affiliation.org}

% \author{Julius P. Kumquat}
% \affiliation{%
%   \institution{The Kumquat Consortium}
%   \city{New York}
%   \country{USA}}
% \email{jpkumquat@consortium.net}


==> imgs/fig1.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=.9\textwidth]{imgs/fig1_pdf.pdf}
    \caption{Images from the same hotel may (left) or may not (right) be connected, while images from different hotels may be connected (middle). Here, we have example images from four different hotels. Images from the same hotel are indicated with the same border color. We see that not all of the images in the same class are connected to each other (only purple class has all the pairwise connections between the examples). We also see that different classes can be connected to each other due to similar features (e.g., red and green class which share the same carpet).}
    \label{fig:image-linking}
\end{figure*}

==> imgs/img-same-chain-diff-label.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.40\linewidth]{imgs/img-same-chain-diff-label_rgb_names_bf_pdf.pdf}
         \vspace{-10pt}
 \caption{Sampled images from Hotels-50K, showcasing 9 \textbf{different} hotel branches (i.e. classes) and 3 hotel chains (i.e. super classes). Hotel branches from the same chain may have shared patterns (e.g. bedsheet styles) which motivates splitting the data by chains to have truly unseen classes. }%For example, this image depicts 9 different branches from three different hotel chains indicated with colors \textcolor{mygreen}{green}, \textcolor{myred}{red}, and \textcolor{myblue}{blue}.}
    % \caption{Different hotels branches from the same chain may have shared patterns (e.g. bedsheet styles). For example, this image depicts 9 different branches from three different hotel chains indicated with colors \textcolor{mygreen}{green}, \textcolor{myred}{red}, and \textcolor{myblue}{blue}.}
    
    \label{fig:hotel-same-chain}
    
\end{figure}
% \vspace{-5ex}

% green: 009900
% red: CC0000
% blue: 000099

==> sections/040experiment.tex <==

% \section{Evaluation and Results}
% \label{sec:res}

% In our experiments, we train baseline models and our method with two general sets of augmentations, \strongaug, which are augmentations that have been finetuned on the target dataset (for \cifarten \cite{krizhevsky2009learning}) or ImageNet in the case of under-studied datasets (for \aircrafts \cite{maji2013fine}, \pathmnist, \tissuemnist, and \hotelsid), and \weakaug, representing the scenario where we do not know the correct augmentations and use minimal augmentations.
% The set of \strongaug consists of \texttt{random-resized-crop}, \texttt{random-horizontal-flip}, \texttt{color-jitter}, \texttt{gray-scale}, \texttt{gaussian-blur} and \texttt{solarization} while \weakaug only uses \texttt{random-horizontal-flip}.


% We choose SimCLR, BYOL, NNCLR, and VICReg as baseline SSL models and couple \ourstrategy with them for comparison. We opted for a \textit{randomly-initialized} backbone conv \cite{he2016deep} as the encoder 
% Note that baseline SSL methods are commonly used for \emph{pre-training} on larges scale datasets, e.g. ImageNet, and learn the the new datasets by transfer learning in the next steps. However, we opt to use \emph{randomly-initialized} backbones to provide a general SSL strategy that can be applied to randomly-initialized encoders to avoid extra pre-training computation.

% % \input{tabs/all-datasets-metrics}
% \input{tabs/hotelid-ssl-metrics}
% \input{tabs/iclr-results}

% \subsection{\strongaug Setting}

% The DA in this configuration consist of strong augmentations that usually distort the size, resolution, and color characteristics of the original image. We see baseline SSL models perform better than \ourmethod on \cifarten, \cifarhundred, and \svhn (Table \ref{tab:all-datasets-metrics}). However, we see the opposite is true for the under-studied and real-word datasets, \aircrafts and \hotelsid (Table \ref{tab:all-datasets-metrics} and \ref{tab:hotelid-ssl-metrics}). The reason for this is that the strong DA have been curated for well-studied datasets, but the optimal set and configuration of DA for one dataset is not necessarily the optimal set and configuration for another. Hence, they do not transfer well to the under-studied datasets. This is where the \ourstrategy complements the strong augmentations and creates better augmentations for the SSL method to learn. Note that \ourmethod also performs comparable to the best-performing baseline SSL model on \cifarten and \cifarhundred as well, i.e., VICReg, meaning \ourmethod does not harm the performance much even if we have the optimal set of strong augmentations. The results for these experiments can be seen in Tables \ref{tab:all-datasets-metrics} and \ref{tab:hotelid-ssl-metrics}.

% Moreover, in Table \ref{tab:hotelid-ssl-metrics}, we observe that the order of best performing SSL models changes among the different evaluation splits, depending on the splits characteristics. This depicts that that our evaluation splits are meaningfully different and for a method should ideally work well on \textit{all} evaluation splits to be used for anti-HT applications. However, the reason \firsttest, consisting of seen classes and super-classes present in the training set, is counter-intuitively more difficult than the rest is because of how the split was constructed; the generally small class size and also the high number of classes (Section \ref{sec:dataset}) causes the retrieval task to be more difficult.

% \subsection{\weakaug Setting}

% We perform all experiments under the \weakaug setting as well, showing \ourstrategy produces high quality approximates for strong augmentations for SSL training. As seen in Tables \ref{tab:all-datasets-metrics} and \ref{tab:hotelid-ssl-metrics}, we see \ourmethod significantly outperforms all methods across both well-studied and under-studied datasets. 

% Furthermore, we see the performance of \ourmethod in the \weakaug setting is comparable to (and in some cases better than) baseline SSL methods in the \strongaug setting on \aircrafts and \hotelsid. Also in Section \ref{sec:ablation}, we also show with a stronger prior knowledge, our method with \weakaug is comparable to SSL methods with \strongaug on \cifarten (Table \ref{tab:cifar10-capacities}). These results show that our \ourstrategy strategy, though conceptually simple, coupled with the \weakaug setting, approximates strong augmentations used in the \strongaug configuration. This creates a significant advantage for \ourmethod to be applied to real-world datasets that strong augmentations have not been studied for them.

% % The increasing difficulty can also be seen for the image retrieval task between \secondtest and \thirdtest. However, the reason \firsttest is counter-intuitively more difficult than the rest, is because of how the split was constructed; the generally small class size and also the high number of classes causes the retrieval task to be more difficult. More information with regard to the datasplit generation can be found in Appendix \ref{app:generation}.

==> sections/080listOfToDo.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AUTHOR: Christos Faloutsos
% INSTITUTION: CMU
% DATE: April 2019
% GOAL: to streamline the paper presentations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\todototoc
\listoftodos

\textcolor{red}{LIST OF TODO}:

Camera version:
\begin{itemize}


    
\item training with random seeds two see which ones perform better
\item evaluating with multiple random seeds for an approximation and getting more robust results
\item training with multiple versions of splits with same characteristics

\item running multiple seeds for more robust experiments, 

\item fix model selection with two different model selection, one for auc one for image retrieval

\end{itemize}

Future: 
\begin{itemize}

\item Think of another domain for the dataset

\item Actually make a dataset with the characteristics we descirbe

\end{itemize}

==> tabs/all-datasets-metrics.tex <==
\begin{table*}[ht!]
\caption{Classification accuracy of \ourmethod and baseline SSL method on four datasets, each in \strongaug and \weakaug setting. The set of DA used for \strongaug are \texttt{random-resized-crop}, \texttt{random-horizontal-flip}, \texttt{color-jitter}, \texttt{gray-scale}, \texttt{gaussian-blur} and \texttt{solarization} and for \weakaug the only DA used is \texttt{random horizontal flip}. We mark the best performing score in \textbf{bold}.}
\begin{center}
 \resizebox{\linewidth}{!}{%
\begin{tabular}{clllllllllllllllll}
    \hline
    \multicolumn{1}{|c}{}    & \multicolumn{4}{c}{\cifarten}            & \multicolumn{4}{c}{\cifarhundred}         & \multicolumn{4}{c}{\svhn} &      \multicolumn{4}{c|}{\aircrafts}            \\
    \hline
    \multicolumn{1}{|c|}{Methods}  &  \weakaug  & \multicolumn{1}{c|}{K} &  \strongaug & \multicolumn{1}{c|}{K} & \weakaug & \multicolumn{1}{c|}{K}  &  \strongaug & \multicolumn{1}{c|}{K} & \weakaug & \multicolumn{1}{c|}{K}   &  \strongaug & \multicolumn{1}{c|}{K}  &    \weakaug & \multicolumn{1}{c|}{K}   &  \strongaug & \multicolumn{1}{c|}{K}  \\
    
    \hline
    \hline
    \multicolumn{1}{|c|}{SimCLR \cite{chen2020simple}}  &   47.62 &  \multicolumn{1}{l|}{1} & 87.57 &  \multicolumn{1}{l|}{1} &       26.14 &  \multicolumn{1}{l|}{1} &  61.57 &  \multicolumn{1}{l|}{1} &      45.35 &  \multicolumn{1}{l|}{1} &  90.94 &  \multicolumn{1}{l|}{1} &  7.70 &  \multicolumn{1}{l|}{1}     &  37.88 &  \multicolumn{1}{l|}{1}      \\           
    \multicolumn{1}{|c|}{BYOL \cite{grill2020bootstrap}}           &   49.72 &  \multicolumn{1}{l|}{1}             &  86.97 &  \multicolumn{1}{l|}{1}             &       29.28 &  \multicolumn{1}{l|}{1} &  59.48 &  \multicolumn{1}{l|}{1} &         43.97 &  \multicolumn{1}{l|}{1} &  87.04 &  \multicolumn{1}{l|}{1} &       8.99 &  \multicolumn{1}{l|}{1}                 &  23.82 &  \multicolumn{1}{l|}{1}                 \\           
    \multicolumn{1}{|c|}{NNCLR \cite{dwibedi2021little}}         &   71.47 &  \multicolumn{1}{l|}{1}     &  86.06 &  \multicolumn{1}{l|}{1}    &          10.90 &  \multicolumn{1}{l|}{1} &  62.46 &  \multicolumn{1}{l|}{1} &         20.08 &  \multicolumn{1}{l|}{1} &  90.85 &  \multicolumn{1}{l|}{1} &  8.10 &  \multicolumn{1}{l|}{1}        &  29.67 &  \multicolumn{1}{l|}{1}        \\  

    \multicolumn{1}{|c|}{Barlow Twins\cite{zbontar2021barlow}}         &   42.00 &  \multicolumn{1}{l|}{1}     &  86.45 &  \multicolumn{1}{l|}{1}    &          - &  \multicolumn{1}{l|}{1} &  - &  \multicolumn{1}{l|}{1} &         35.91 &  \multicolumn{1}{l|}{1} &  91.71 &  \multicolumn{1}{l|}{1} &  7.53 &  \multicolumn{1}{l|}{1}        &  17.67 (24.45) &  \multicolumn{1}{l|}{1}        \\  
    
    \multicolumn{1}{|c|}{VICReg \cite{bardes2021vicreg}}   &   36.04 &  \multicolumn{1}{l|}{1}                       &  \textbf{89.92} &  \multicolumn{1}{l|}{1}                       &         22.80 &  \multicolumn{1}{l|}{1} &  \textbf{66.41} &  \multicolumn{1}{l|}{1} &   26.29 &  \multicolumn{1}{l|}{1} &  \textbf{91.94} &  \multicolumn{1}{l|}{1} &      4.95 &  \multicolumn{1}{l|}{1}        &  19.02 &  \multicolumn{1}{l|}{1} \\           
    \hline
    \multicolumn{1}{|c|}{\oursimclr (ours)}    &   \textbf{73.81} &  \multicolumn{1}{l|}{10}             &  85.53 &  \multicolumn{1}{l|}{2}             &        \textbf{52.32} &  \multicolumn{1}{l|}{1} &  59.21 &  \multicolumn{1}{l|}{1} &            \textbf{61.05} &  \multicolumn{1}{l|}{5} &  83.80 &  \multicolumn{1}{l|}{2} &  18.15 &  \multicolumn{1}{l|}{10}                 &  \textbf{39.84} &  \multicolumn{1}{l|}{2}               \\                   
    
    \multicolumn{1}{|c|}{\ourbyol (ours)}    &   74.04 &  \multicolumn{1}{l|}{10}             &  83.51 &  \multicolumn{1}{l|}{2}             &        52.00 &  \multicolumn{1}{l|}{1} &  56.33 &  \multicolumn{1}{l|}{1} &            64.47 &  \multicolumn{1}{l|}{2} &  66.41 &  \multicolumn{1}{l|}{2} &  15.96 &  \multicolumn{1}{l|}{10}                 &  25.17 &  \multicolumn{1}{l|}{2}               \\  
    
    \multicolumn{1}{|c|}{\ourbarlow (ours)}    &   74.24 &  \multicolumn{1}{l|}{10}             &  81.93 &  \multicolumn{1}{l|}{2}             &        - &  \multicolumn{1}{l|}{1} &  - &  \multicolumn{1}{l|}{1} &            \textbf{60.79} &  \multicolumn{1}{l|}{2} &  80.19 &  \multicolumn{1}{l|}{2} &  16.26 &  \multicolumn{1}{l|}{10}                 &  20.91 (31.05) &  \multicolumn{1}{l|}{5}               \\                   

    \multicolumn{1}{|c|}{\ourvicreg (ours)}    &   72.60 &  \multicolumn{1}{l|}{10}             &  85.54 &  \multicolumn{1}{l|}{2}             &        - &  \multicolumn{1}{l|}{1} &  - &  \multicolumn{1}{l|}{1} &  57.48 &  \multicolumn{1}{l|}{5}                 &  87.00 &  \multicolumn{1}{l|}{2} &            \textbf{19.26} &  \multicolumn{1}{l|}{10} &  39.87 &  \multicolumn{1}{l|}{5}               \\                   

    
    \hline
\end{tabular}
}





%  \resizebox{\linewidth}{!}{%
% \begin{tabular}{clllllllll}
%     \hline
%     \multicolumn{1}{|c}{}    & \multicolumn{2}{c}{\cifarten}            & \multicolumn{2}{c}{\cifarhundred}         & \multicolumn{2}{c}{\svhn} &      \multicolumn{2}{c|}{\aircrafts}            \\
%     \hline
%     \multicolumn{1}{|c|}{Methods}  &  \weakaug   &  \multicolumn{1}{c|}{\strongaug} & \weakaug  &  \multicolumn{1}{c|}{\strongaug} & \weakaug   &  \multicolumn{1}{c|}{\strongaug}  &    \weakaug   &  \multicolumn{1}{c|}{\strongaug}  \\
    
%     \hline
%     \hline
%     \multicolumn{1}{|c|}{SimCLR \cite{chen2020simple}}  &   47.62 &  \multicolumn{1}{l|}{87.57} &       26.14 &  \multicolumn{1}{l|}{61.57} &      45.35 &  \multicolumn{1}{l|}{90.94} &  7.70     &  \multicolumn{1}{l|}{37.88}      \\           
%     \multicolumn{1}{|c|}{BYOL \cite{grill2020bootstrap}}           &   49.72             &  \multicolumn{1}{l|}{86.97}             &       29.28 &  \multicolumn{1}{l|}{59.48} &         43.97 &  \multicolumn{1}{l|}{87.04} &       8.99                 &  \multicolumn{1}{l|}{23.82}                 \\           
%     \multicolumn{1}{|c|}{NNCLR \cite{dwibedi2021little}}         &   71.47     &  \multicolumn{1}{l|}{86.06}    &          10.90 &  \multicolumn{1}{l|}{62.46} &         20.08 &  \multicolumn{1}{l|}{90.85} &  8.10        &  \multicolumn{1}{l|}{29.67}        \\     
    
%     \multicolumn{1}{|c|}{VICReg \cite{bardes2021vicreg}}   &   36.04                       &  \multicolumn{1}{l|}{\textbf{89.92}}                       &         22.80 &  \multicolumn{1}{l|}{\textbf{66.41}} &   26.29 &  \multicolumn{1}{l|}{\textbf{91.94}} &      4.95        &  \multicolumn{1}{l|}{19.02} \\           
%     \hline
%     \multicolumn{1}{|c|}{\ourmethod (ours)}    &   \textbf{73.81}             &  \multicolumn{1}{l|}{85.53}             &        \textbf{52.32} &  \multicolumn{1}{l|}{59.21} &            \textbf{61.05} &  \multicolumn{1}{l|}{83.80} &  \textbf{18.15}                 &  \multicolumn{1}{l|}{\textbf{39.84}}               \\                   
%     \hline
% \end{tabular}
% }
\end{center}
\label{tab:all-datasets-metrics-200eps}
\end{table*}


==> tabs/before_after_hotel.tex <==
% \begin{table}[]
% \caption{Number of images, branches (classes), and chains (super-classes) in the original and cleaned version of the dataset.}
% \label{tab:before-after-hotels}
% \small
% \begin{tabular}{c|ccc}
% \small
%       & Images & Branches & Chains \\ \hline
% Hotels-50K Original & 1,140,383    & 50,000         & 91           \\
% Hotels-50K Cleaned  & 1,071,953    & 45,438         & 91          \\
% Hotels-ID  & 97,553    & 7,769   & 87         
% \end{tabular}
% \end{table}

% %  images from 


\begin{table}[]
% \vspace{-10pt}
\caption{Number of images, branches (classes), and chains (super-classes) in the original and cleaned version of the dataset.}
\label{tab:before-after-hotels}
\small
\begin{tabular}{c|ccc}
\small
       & Images & Branches & Chains \\ \hline
Hotels-50K & 1,140,383    & 50,000         & 91           \\
\hotelsfifty  & 1,071,953    & 45,438         & 91          \\
\hotelsid  & 97,553    & 7,769   & 87         
\end{tabular}
\end{table}

%  images from 

==> tabs/cifar10-capacities.tex <==
\begin{table}[ht!]
\caption{Classification accuracy of \ourmethod with three different prior knowledge models ($PK$-model) on \cifarten and \aircrafts in \strongaug and \weakaug settings. We show whether the $PK$-model was pretrained using CLIP (-CLIP) or supervised training (-SUP). We mark the best performing score in \textbf{bold}.}
\begin{center}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cclllll}
            \hline
             \multicolumn{1}{|c}{}    &     &    \multicolumn{2}{c}{\cifarten}         &   \multicolumn{2}{c|}{\aircrafts}            \\
            \hline
            \multicolumn{1}{|c}{Methods}  & \multicolumn{1}{c|}{$PK$-Model} &    \weakaug   &  \multicolumn{1}{c|}{\strongaug} & \weakaug  &  \multicolumn{1}{c|}{\strongaug}  \\
            \hline
            \hline
            % \multicolumn{1}{|c|}{SimCLR \cite{chen2020simple}}  &   47.62 &  \multicolumn{1}{l|}{87.57} &       26.14 &  \multicolumn{1}{l|}{61.57} &      45.35 &  \multicolumn{1}{l|}{90.94} &  7.70     &  \multicolumn{1}{l|}{37.88}      \\           
            \multicolumn{1}{|c}{\multirow{3}{*}{$\ourmethod$}}    &   \multicolumn{1}{c|}{RN18-SUP}     &     73.81                 &       \multicolumn{1}{c|}{85.53}                  &       18.15                &       \multicolumn{1}{c|}{39.84}   \\
            \multicolumn{1}{|c}{}    &   \multicolumn{1}{c|}{RN50-SUP}    &   77.97                 &        \multicolumn{1}{c|}{86.82}                 &       15.66                &       \multicolumn{1}{c|}{38.63}  \\
            \multicolumn{1}{|c}{}    &  \multicolumn{1}{c|}{RN50-CLIP}    &   \textbf{86.95}                  &       \multicolumn{1}{c|}{\textbf{89.62}}                  &       \textbf{20.55}                &       \multicolumn{1}{c|}{\textbf{44.10}}  \\
            \hline
        \end{tabular}
    }
\end{center}
\label{tab:cifar10-capacities}
\end{table}


==> tabs/hid-fig-table.tex <==
\begin{minipage}{\textwidth}
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=1.0\linewidth]{imgs/img-same-chain-diff-label_rgb_names_bf_pdf.pdf}
         \vspace{-10pt}
     \captionof{figure}{ 
    Images from Hotel-ID, showcasing 9 distinct hotel branches within 3 chains. We separate the data by chains to introduce \textit{genuinely} new classes due to shared patterns within the same chain.
     % Sampled images from Hotels-50K, showcasing 9 \textbf{different} hotel branches (i.e. classes) and 3 hotel chains (i.e. super classes). Hotel branches from the same chain may have shared patterns (e.g. bedsheet styles) which motivates splitting the data by chains to have truly unseen classes. 
     }
     
     
     %For example, this image depicts 9 different branches from three different hotel chains indicated with colors \textcolor{mygreen}{green}, \textcolor{myred}{red}, and \textcolor{myblue}{blue}.}
    % \caption{Different hotels branches from the same chain may have shared patterns (e.g. bedsheet styles). For example, this image depicts 9 different branches from three different hotel chains indicated with colors \textcolor{mygreen}{green}, \textcolor{myred}{red}, and \textcolor{myblue}{blue}.}
    
    \label{fig:hotel-same-chain}\vspace{-14ex} 
  \end{minipage}
  \hspace{4pt}
  \resizebox{0.5\textwidth}{!}{
  \begin{minipage}[b]{0.54\textwidth}
    \centering
    \captionof{table}{\recallatone on different spltis on \hotelsid Dataset for SSL methods. The splits are namely, \firsttest: \{branch: seen, chain: seen\}, \secondtest: \{branch: unseen, chain: seen\}, \thirdtest: \{branch: unseen, chain: unseen\} and  \fourthtest: \{branch: unknown, chain: unknown\}.  We mark the \FB{first}, \SB{second}, and \TB{third} best results accordingly.
    % \af{add filler to align table with figure, or reduce figure caption}
    }
    \label{tab:hotelid-ssl-metrics}
    
        \begin{tabular}{clllll}
            % \toprule
            % \multicolumn{1}{c}{}    &  \multicolumn{4}{c}{\hotelsid} \\
            \toprule
            \multicolumn{1}{c}{\textbf{Method}}   & \firsttest            &      \secondtest           &   {\thirdtest}             &       \multicolumn{1}{c}{\fourthtest}      \\
            \bottomrule
            \toprule
            \multicolumn{1}{c}{{SimCLR}}    &   \multicolumn{1}{|c}{3.28} &        16.76         &       20.30         &       \multicolumn{1}{c}{16.00}    \\    
        
            
            \multicolumn{1}{c}{{BYOL}}           &   \multicolumn{1}{|c}{3.69}                       &       19.27                           &       23.02      &       \multicolumn{1}{c}{18.47}   \\           

            \multicolumn{1}{c}{{Barlow Twins}}         &   \multicolumn{1}{|c}{3.04}    &       15.54               &       18.96            &       \multicolumn{1}{c}{15.06}   \\    
            

            \multicolumn{1}{c}{{VICReg}}   &   \multicolumn{1}{|c}{3.41}        &       17.52                  &        20.45            &       \multicolumn{1}{c}{16.53}  \\        

            \midrule
            
            \multicolumn{1}{c}{$\oursimclr$ (ours)}    &   \multicolumn{1}{|c}{\SB{4.84}}                 &        \SB{23.67}                 &       \SB{26.30}                &       \multicolumn{1}{c}{\SB{22.28}}  \\
            \multicolumn{1}{c}{$\ourbyol$ (ours)}    &   \multicolumn{1}{|c}{3.89}                 &        19.64                 &       23.18                &       \multicolumn{1}{c}{19.38}  \\
            \multicolumn{1}{c}{$\ourbarlow$ (ours)}    &   \multicolumn{1}{|c}{\TB{4.49}}                 &        \TB{21.98}                 &       \TB{25.23}                &       \multicolumn{1}{c}{\TB{20.82}}  \\
            \multicolumn{1}{c}{$\ourvicreg$ (ours)}    &   \multicolumn{1}{|c}{\FB{5.33}}                 &        \FB{25.71}                 &       \FB{28.29}                &       \multicolumn{1}{c}{\FB{23.78}}  \\            
            \bottomrule
        \end{tabular}

    \end{minipage}
    }
    

\end{minipage}
\vspace{2.5ex} 

==> tabs/hotelid-capacities.tex <==
\begin{table}[ht!]
\caption{\recallatone performance of of BYOL combined with \ourstrategy (PK-BYOL) and also with different pretrained models as prior knowledge ($PK$-Model) evaluated on \hotelsid splits. We mark the best performing score in \textbf{bold}.}
\begin{center}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{ccc|lllll}
            \hline
            \multicolumn{3}{|c}{}    &  \multicolumn{4}{c|}{\hotelsid} \\
            \hline
            \multicolumn{1}{|c}{Method}  &  DA   &   $PK$-Model   &  \firsttest            &      \secondtest           &   {\thirdtest}             &       \multicolumn{1}{c|}{\fourthtest}      \\
            \hline
            \hline
            \multicolumn{1}{|c}{\multirow{2}{*}{$\ourmethod$}}    &  \multirow{2}{*}{\strong} & RN50     &     \textbf{4.29}                 &       \textbf{21.18}                  &       \textbf{23.77}                &       \multicolumn{1}{c|}{\textbf{19.82}}   \\
            \multicolumn{1}{|c}{}    &   & RN18    &   4.09                 &        19.55                 &       22.85                &       \multicolumn{1}{c|}{18.68}  \\
            \hline 
            \multicolumn{1}{|c}{\multirow{2}{*}{$\ourmethod$}}    &  \multirow{2}{*}{\weak} & RN50    &   2.57                  &       14.34                  &       17.67                &       \multicolumn{1}{c|}{14.13} \\
            \multicolumn{1}{|c}{}    &    & RN18    &   2.95                  &       15.00                  &       17.77                &       \multicolumn{1}{c|}{15.26}  \\
            \hline 
            \multicolumn{1}{|c}{\multirow{2}{*}{\ourbyol}}    &  \strong & RN50      &   2.84                  &       13.93                  &       17.80                &       \multicolumn{1}{c|}{14.30}   \\          
             \multicolumn{1}{|c}{}  &  \weak & RN50      &   2.90                  &       14.89                  &       18.27                &       \multicolumn{1}{c|}{14.62}   \\          
            \hline
        \end{tabular}
    }
\end{center}
\label{tab:hotelid-capacities}
\end{table}


==> tabs/hotelid-splits.tex <==
% \begin{table}[]
% \caption{Proposed splits for Hotel-ID number of branches (classes) and chains in each data split.}
% \label{tab:hotelid-splits}
% \begin{tabular}{c|cccc}
%       & Images  & Branches & Chains & \begin{tabular}[c]{@{}c@{}}Avg No. \\  Images Per Class\end{tabular} \\ \hline
% Train  & 29,326 & 3,150   & 65     & 9.31
%                 \\
% Trainval  & 46,237 & 4,406   & 75     & 10.49
%                 \\ \hline
% Val 1  & 3,704  & 1,033    & 57     & 3.59                                                                 \\
% Test 1 & 9,013  & 3,698   & 74     & 4.45                                                                 \\ \hline
% Val 2  & 6,612  & 617      & 56     & 10.72                                                                \\
% Test 2 & 11,110  & 881    & 61     & 12.61                                                                \\ \hline
% Val 3  & 6,595  & 639      & 10      & 10.32                         
%                     q\\
% Test 3 & 10,973  & 737    & 12      & 14.89
% \\ \hline
% % Val 4  & 17,981  & 702      & -      & 25.61                                                                \\
% Test 4 & 20,220   & 1,745    & -      & 11.59
% \\ \hline
% Total & 97,553   & 7,769     & 87      & 12.56
                                                               
% \end{tabular}
% \end{table}


\begin{table}[]
\centering
\caption{\hotelsid: proposed splits for Hotel-ID number of branches (classes) and chains (super-classes) in each data split.}
\label{tab:hotelid-splits}
\small
    \begin{tabular}{c|ccc}
       & Images  & Branches & Chains \\ \midrule
        Train  & 29,326 & 3,150   & 65     
                        \\
        Trainval  & 46,237 & 4,406   & 75     
                        \\ \midrule
        \firstval  & 3,704  & 1,033    & 57     
        \\
        \firsttest & 9,013  & 3,698   & 74                                                                      \\ \midrule
        \secondval  & 6,612  & 617      & 56                                                                    \\
        \secondtest & 11,110  & 881    & 61                                                                     \\ \midrule
        \thirdval  & 6,595  & 639      & 10                               
                            \\
        \thirdtest & 10,973  & 737    & 12      
        \\ \midrule
        
        \fourthtest & 20,220   & 1,745    & -    
        \\ \midrule
        Total & 97,553   & 7,769     & 87    
                                                                       
        \end{tabular}
        \label{tab:hotelid-splits}
\end{table}

==> tabs/hotels-explain.tex <==
\begin{table}
\begin{center}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{cccc}
\hline
 & \textbf{\firsttest} & \textbf{\secondtest} & \textbf{\thirdtest} \\
\hline
\textbf{Train set} & \textbf{Shared branches (classes)}\textbf{and shared chains (super-classes)} & \textbf{Only shared chains (super-classes)}

\textbf{branches are distinct} & \textbf{Both chains and branches are distinct.} \\
\hline

\end{tabular}
}
\end{center}

\end{table}


==> tabs/hotels-splits.tex <==
% \begin{table}[]
% \caption{Proposed splits with the number of branches (classes) and chains in each data split.}
% \label{tab:hotels-splits}
% \begin{tabular}{c|ccc}
%       & Images  & Branches & Chains \\ \hline
% Train  & 294,275 & 17,281   & 81     \\ \hline
% Val 1  & 22,121  & 4,941    & 79     \\
% Test 1 & 51,294  & 11,532   & 81     \\ \hline
% Val 2  & 16,095  & 740      & 71     \\
% Test 2 & 36,537  & 1,728    & 79     \\ \hline
% Val 3  & 15,970  & 897      & 3      \\
% Test 3 & 35,693  & 1,365    & 7      \\ \hline
% Val 4  & 17,981  & 702      & -      \\
% Test 4 & 41,437  & 1,640    & -     
% \end{tabular}
% \end{table}


% \begin{table}[]
% \caption{Proposed splits with the number of branches (classes) and chains in each data split.}
% \label{tab:hotels-splits}
% \begin{tabular}{c|cccc}
%       & Images  & Branches & Chains & \begin{tabular}[c]{@{}c@{}}Avg No. \\  Images Per Class\end{tabular} \\ \hline
% Train  & 294,275 & 17,281   & 81     & 17.03                                                                \\
% Trainval & 348,461 & 18,918 & 84 & 18.42 
%                             \\ \hline
% Val 1  & 22,121  & 4,941    & 79     & 4.48                                                                 \\
% Test 1 & 51,294  & 11,532   & 81     & 4.45                                                                 \\ \hline
% Val 2  & 16,095  & 740      & 71     & 21.75                                                                \\
% Test 2 & 36,537  & 1,728    & 79     & 21.14                                                                \\ \hline
% Val 3  & 15,970  & 897      & 3      & 17.8                                                                 \\
% Test 3 & 35,693  & 1,365    & 7      & 26.15                                                                \\ \hline
% % Val 4  & 17,981  & 702      & -      & 25.61                                                                \\
% Test 4 & 41,437  & 1,640    & -      & 25.27                                                               
% \end{tabular}
% \end{table}

\begin{table}[]
\vspace{-15pt}
\centering
\caption{\hotelsfifty: proposed splits with the number of branches (classes) and chains in each data split which determine four different settings explained in Figure \ref{fig:hotels50k-auc-barplot}.% \firsttest: \{branch: seen, chain: seen\}, \secondtest: \{branch: unseen, chain: seen\}, \thirdtest: \{branch: unseen, chain: unseen\}, \fourthtest: \{branch: unknown, chain: unknown\}.
}
\label{tab:hotels-splits}
\small
\begin{tabular}{c|ccc}
       & Images  & Branches & Chains \\ \hline
Train  & 294,275 & 17,281   & 81                                                                \\
Trainval & 348,461 & 18,918 & 84
                            \\ \hline
\firstval  & 22,121  & 4,941    & 79                                                                 \\
\firsttest & 51,294  & 11,532   & 81                                                                 \\ \hline
\secondval  & 16,095  & 740      & 71                                                                \\
\secondtest & 36,537  & 1,728    & 79                                                                \\ \hline
\thirdval  & 15,970  & 897      & 3                                                                  \\
\thirdtest & 35,693  & 1,365    & 7                                                                 \\ \hline
% Val 4  & 17,981  & 702      & -                                                                    \\
\fourthtest & 41,437  & 1,640    & -   \\ \hline
Total & 471,985 & 35,003 & 91
\end{tabular}\vspace{-10pt}
\end{table}

==> tabs/hyperparams.tex <==
\begin{table}[ht]
\caption{Final hyper-parameters chosen for each dataset. This the columns represent the learning rate (LR), batch size (BS), and other hyper-parameters specific to the method, namely proxy learning rate (plr), centers per class (clc), temperature (temp), and number of classes per batch (nc). }
\begin{center}
 \resizebox{0.99\linewidth}{!}{%
\begin{tabular}{cllllll}
    \hline
    \multicolumn{1}{|c}{}    & \multicolumn{3}{c}{\hotelsfifty}            &      \multicolumn{3}{c|}{\hotelsid}      \\
    \hline
    \multicolumn{1}{|c|}{Hyper Parameters}  &  LR   &   BS   &  \multicolumn{1}{c|}{Other} & LR   &   BS   &  \multicolumn{1}{c|}{Other}  \\
    \hline
    \hline
    \multicolumn{1}{|c|}{Triplet \cite{weinberger2006distance}}  &   0.00001   &   80   &  \multicolumn{1}{l|}{-}     &       0.00003   &   80   &  \multicolumn{1}{l|}{-}    \\
    \multicolumn{1}{|c|}{Circle \cite{sun2020circle}}  &   0.0001   &   80   &  \multicolumn{1}{l|}{-}     &       0.0001   &   80   &  \multicolumn{1}{l|}{-}    \\
    \multicolumn{1}{|c|}{MultiSim \cite{wang2019multi}}    &   0.00003   &   80   &  \multicolumn{1}{l|}{-}     &       0.0001   &   256   &  \multicolumn{1}{l|}{-}    \\ 
    \multicolumn{1}{|c|}{ProxyNCA++ \cite{teh2020proxynca++}}  &   0.024   &   96   &  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}plr: 240\\ nc: 32\end{tabular}}     &       0.024   &   192   &  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}} plr: 240\\ nc: 64\end{tabular}}  \\
    \multicolumn{1}{|c|}{SupCon \cite{khosla2020supervised}}   &    0.00001   &   80   &  \multicolumn{1}{l|}{temp: 0.05}     &       0.00003   &   256   &  \multicolumn{1}{l|}{temp: 0.05}    \\
    \multicolumn{1}{|c|}{SoftTriple \cite{qian2019softtriple}}    &   0.00003   &   64   &  \multicolumn{1}{l|}{cpc: 5}     &       0.00003   &   64   &  \multicolumn{1}{l|}{cpc: 20}    \\
    \multicolumn{1}{|c|}{BCE}       &   0.0003   &   80   &  \multicolumn{1}{l|}{-}     &        0.0001   &   128   &  \multicolumn{1}{l|}{-}    \\
    \multicolumn{1}{|c|}{Hard BCE}    &    0.00001   &   80   &  \multicolumn{1}{l|}{-}     &        0.0001   &   256   &  \multicolumn{1}{l|}{-}    \\
    \hline
\end{tabular}
}
\end{center}
\label{tab:hyperparams}
\end{table}
% \cline{1-2}


==> tabs/iclr-results-k.tex <==
\begin{table*}[ht!]
\caption{Classification accuracy of \ourmethod and baseline SSL method on four datasets, each in \strongaug and \weakaug setting. The set of DA used for \strongaug are \texttt{random-resized-crop}, \texttt{random-horizontal-flip}, \texttt{color-jitter}, \texttt{gray-scale}, \texttt{gaussian-blur} and \texttt{solarization} and for \weakaug the only DA used is \texttt{random horizontal flip}. We mark the best performing score in \textbf{bold}.}
\begin{center}
 \resizebox{\linewidth}{!}{%
\begin{tabular}{clllllllllllllllll}
    \hline
    \multicolumn{1}{|c}{}           & \multicolumn{2}{c}{\cifarten}            & \multicolumn{2}{c}{\aircrafts}         & \multicolumn{2}{c}{\pathmnist} &      \multicolumn{2}{c|}{\tissuemnist}            \\
    \hline
    \multicolumn{1}{|c|}{Methods}  &  \strongaug & \multicolumn{1}{c|}{K}  &  \strongaug & \multicolumn{1}{c|}{K}  &  \strongaug & \multicolumn{1}{c|}{K} &  \strongaug & \multicolumn{1}{c|}{K}  \\
    
    \hline
    \hline
    \multicolumn{1}{|c|}{SimCLR}            &  88.26          &  \multicolumn{1}{l|}{1}     &  39.27    &  \multicolumn{1}{l|}{1} &  91.56         &  \multicolumn{1}{l|}{1}    &  61.51 &  \multicolumn{1}{l|}{1}   \\           
    \multicolumn{1}{|c|}{BYOL}              &  -----          &  \multicolumn{1}{l|}{1}     &  -----    &  \multicolumn{1}{l|}{1} &  91.24         &  \multicolumn{1}{l|}{1}    &  60.73 &  \multicolumn{1}{l|}{1}   \\           
    \multicolumn{1}{|c|}{NNCLR}             &  -----          &  \multicolumn{1}{l|}{1}     &  -----    &  \multicolumn{1}{l|}{1} &  -----         &  \multicolumn{1}{l|}{1}    &  ----- &  \multicolumn{1}{l|}{1}   \\  
    \multicolumn{1}{|c|}{Barlow Twins}      &  88.89          &  \multicolumn{1}{l|}{1}     &  -----    &  \multicolumn{1}{l|}{1} &  92.23         &  \multicolumn{1}{l|}{1}    &  60.06 &  \multicolumn{1}{l|}{1}   \\  
    \multicolumn{1}{|c|}{VICReg}            &  89.34          &  \multicolumn{1}{l|}{1}     &  33.21    &  \multicolumn{1}{l|}{1} &  92.27         &  \multicolumn{1}{l|}{1}    &  59.41 &  \multicolumn{1}{l|}{1}   \\           
    \hline
    \multicolumn{1}{|c|}{\oursimclr (ours)} &  89.57          &  \multicolumn{1}{l|}{2}     &  49.57    &  \multicolumn{1}{l|}{1} & \textbf{92.19} &  \multicolumn{1}{l|}{5}    &  62.76 &  \multicolumn{1}{l|}{2}   \\                   
    
    \multicolumn{1}{|c|}{\ourbyol (ours)}   &  -----          &  \multicolumn{1}{l|}{2}     &  45.48    &  \multicolumn{1}{l|}{1} & 91.05          &  \multicolumn{1}{l|}{2}    &  54.05 &  \multicolumn{1}{l|}{2}   \\  
    
    \multicolumn{1}{|c|}{\ourbarlow (ours)} &  88.39          &  \multicolumn{1}{l|}{2}     &  -----    &  \multicolumn{1}{l|}{1} & 91.55          &  \multicolumn{1}{l|}{2}    &  62.93 &  \multicolumn{1}{l|}{2}   \\                   

    \multicolumn{1}{|c|}{\ourvicreg (ours)} &  89.68          &  \multicolumn{1}{l|}{2}     &  -----    &  \multicolumn{1}{l|}{1} & 91.88          &  \multicolumn{1}{l|}{5}    &  62.46 &  \multicolumn{1}{l|}{2}   \\                   

    
    \hline
\end{tabular}
}
\end{center}
\label{tab:all-datasets-metrics}
\end{table*}


==> tabs/iclr-results-ma.tex <==

\begin{table*}[t]
\caption{Classification accuracy of baseline SSL methods with and without \ourstrategy on four datasets. We consider both \strongaug (Strong Augumentation) and \weakaug (Weak Augumentation), settings. The set of DA used for \strongaug are \texttt{random-resized-crop}, \texttt{random-horizontal-flip}, \texttt{color-jitter}, \texttt{gray-scale}, \texttt{gaussian-blur} and \texttt{solarization}. For the \weakaug setting, the only DA used is \texttt{random horizontal flip}. We mark the \FB{first}, \SB{second} and \TB{third} best performing models accordingly.}
\begin{center}
% \begin{tabular}{cllllllllllll}
\resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|ccccc|}
\begin{tabular}{ccccccc}
    \toprule
     \multirow{3}{*}{\textbf{Aug.}} & \multirow{3}{*}{\textbf{Prior Knwlg.}} & \multirow{3}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Datasets}} \\ \cmidrule{4-7}
    & & \multicolumn{1}{c}{}           & \cifarten            & \aircrafts         & \pathmnist &      \multicolumn{1}{c}{\tissuemnist}            \\
    & & \multicolumn{1}{c}{}           &    \small{(10 classes)}         &    \small{(100 classes)}      & \small{(9 classes)} &  \small{(8 classes)}                \\
    
    \bottomrule
    \toprule
    % WEAK AUG
    \multirow{9}{*}{\rotatebox{90}{\weakaug}} & \multirow{5}{*}{---} &  \multicolumn{1}{c|}{SimCLR}            & 47.62              &  7.70           & 62.99            &  \multicolumn{1}{c}{52.30}            \\           
    & & \multicolumn{1}{c|}{BYOL}              & 49.72              &  8.99           & 77.77            &  \multicolumn{1}{c}{51.00}            \\           
    & & \multicolumn{1}{c|}{NNCLR}             & 71.74              &  8.10           & 56.92            &  \multicolumn{1}{c}{42.59}            \\  
    & & \multicolumn{1}{c|}{Barlow Twins}      & 42.00              &  7.53           & 64.82            &  \multicolumn{1}{c}{49.43}            \\  
    & & \multicolumn{1}{c|}{VICReg}            & 36.04              &  4.95           & 56.92            &  \multicolumn{1}{c}{50.26}            \\ \cmidrule{2-7} 
     & \multirow{4}{*}{$RN18_{SUP}$} & \multicolumn{1}{c|}{\oursimclr (ours)} & \TB{73.81}         &  \SB{18.15}     & \SB{86.98}       &  \multicolumn{1}{c}{\TB{57.62}}            \\                   
    & & \multicolumn{1}{c|}{\ourbyol (ours)}   & \SB{74.04}         &  15.96          & \FB{87.56}       &  \multicolumn{1}{c}{\FB{59.15}}        \\  
    & & \multicolumn{1}{c|}{\ourbarlow (ours)} & \FB{74.24}         &  \TB{16.26}     & 85.08            &  \multicolumn{1}{c}{\SB{58.55}}            \\                   
    & & \multicolumn{1}{c|}{\ourvicreg (ours)} & 72.60              &  \FB{19.26}     & \TB{85.36}       &  \multicolumn{1}{c}{57.06}            \\ \midrule \midrule
     % \cmidrule{1-9}
    % STRONG AUG
     \multirow{9}{*}{\rotatebox{90}{\strongaug}} & \multirow{5}{*}{---} & \multicolumn{1}{c|}{SimCLR}            & 88.26              &  \TB{39.27}          &  91.56           &  \multicolumn{1}{c}{61.51}            \\           
    & & \multicolumn{1}{c|}{BYOL}              & 86.90              &  27.33          &  91.24           &  \multicolumn{1}{c}{60.73}            \\           
    & & \multicolumn{1}{c|}{NNCLR}             & 87.95              &  39.12          &  91.14           &  \multicolumn{1}{c}{52.42}            \\  
    & & \multicolumn{1}{c|}{Barlow Twins}      & 88.89              &  25.71          & \SB{92.23}       &  \multicolumn{1}{c}{60.06}            \\  
    & & \multicolumn{1}{c|}{VICReg}            & \TB{89.34}         &  33.21          & \FB{92.27}       &  \multicolumn{1}{c}{59.41}               \\ \cmidrule{2-7}
     & \multirow{4}{*}{$RN50_{CLIP}$} & \multicolumn{1}{c|}{\oursimclr (ours)} & \SB{89.57}         &  \FB{49.57}     & \TB{92.19}       &  \multicolumn{1}{c}{\TB{62.76}}            \\                   
    & & \multicolumn{1}{c|}{\ourbyol (ours)}   & 88.46              &  32.07     & 91.05            &  \multicolumn{1}{c}{54.05}                 \\  
    & & \multicolumn{1}{c|}{\ourbarlow (ours)} & 88.39              &  25.35          & 91.55            &  \multicolumn{1}{c}{\FB{62.93}}            \\                   
    & & \multicolumn{1}{c|}{\ourvicreg (ours)} & \FB{89.68}         &  \SB{45.48}          & 91.88            &  \multicolumn{1}{c}{\SB{62.46}}            \\ \bottomrule
\end{tabular}
}
\end{center}
    
% \label{tab:all-datasets-metrics-sa}
\label{tab:all-datasets-metrics}
\end{table*}




==> tabs/iclr-results-sa.tex <==
% \begin{table*}[t]
% \caption{{\bf Left:}Classification accuracy of \ourmethod and baseline SSL method on four datasets, in \strongaug setting. The set of DA used for \strongaug are \texttt{random-resized-crop}, \texttt{random-horizontal-flip}, \texttt{color-jitter}, \texttt{gray-scale}, \texttt{gaussian-blur} and \texttt{solarization}. We mark the \FB{first}, \SB{second} and \TB{third} best performing models accordingly.{\bf Right:} Classification accuracy of \ourmethod and baseline SSL method on four datasets, in \weakaug setting. The set of DA used for \weakaug the only DA used is \texttt{random horizontal flip}. We mark the \FB{first}, \SB{second} and \TB{third} best performing models accordingly.}
% \begin{center}
%  \resizebox{0.49\linewidth}{!}{%
% % \begin{tabular}{cllllllllllll}
% \begin{tabular}{ccccc}
%     \hline
%     \multicolumn{1}{|c}{}           & \cifarten            & \aircrafts         & \pathmnist &      \multicolumn{1}{c|}{\tissuemnist}            \\
%     \hline
%     \hline
%     \multicolumn{1}{|c|}{SimCLR}            & 88.26              &  39.27          &  91.56           &  \multicolumn{1}{c|}{61.51}            \\           
%     \multicolumn{1}{|c|}{BYOL}              & 86.90              &  -----          &  91.24           &  \multicolumn{1}{c|}{60.73}            \\           
%     \multicolumn{1}{|c|}{NNCLR}             & 87.95              &  -----          &  91.14           &  \multicolumn{1}{c|}{-----}            \\  
%     \multicolumn{1}{|c|}{Barlow Twins}      & 88.89              &  -----          & \SB{92.23}       &  \multicolumn{1}{c|}{60.06}            \\  
%     \multicolumn{1}{|c|}{VICReg}            & \TB{89.34}         &  33.21          & \FB{92.27}       &  \multicolumn{1}{c|}{59.41}               \\ \hline
%     \multicolumn{1}{|c|}{\oursimclr (ours)} & \SB{89.57}         &  \FB{49.57}     & \TB{92.19}       &  \multicolumn{1}{c|}{\TB{62.76}}            \\                   
%     \multicolumn{1}{|c|}{\ourbyol (ours)}   & 88.46              &  \SB{45.48}     & 91.05            &  \multicolumn{1}{c|}{54.05}                 \\  
%     \multicolumn{1}{|c|}{\ourbarlow (ours)} & 88.39              &  -----          & 91.55            &  \multicolumn{1}{c|}{\FB{62.93}}            \\                   
%     \multicolumn{1}{|c|}{\ourvicreg (ours)} & \FB{89.68}         &  -----          & 91.88            &  \multicolumn{1}{c|}{\SB{62.46}}            \\ \hline
% \end{tabular}
% }
% \resizebox{0.49\linewidth}{!}{%
% % \begin{tabular}{cllllllllllll}
% \begin{tabular}{ccccc}
%     \hline
%     \multicolumn{1}{|c}{}           & \cifarten            & \aircrafts         & \pathmnist &      \multicolumn{1}{c|}{\tissuemnist}            \\
%     \hline
%     \hline
%     \multicolumn{1}{|c|}{SimCLR}            & 47.62              &  7.70           & 62.99            &  \multicolumn{1}{c|}{52.30}            \\           
%     \multicolumn{1}{|c|}{BYOL}              & 49.72              &  8.99           & -----            &  \multicolumn{1}{c|}{51.00}            \\           
%     \multicolumn{1}{|c|}{NNCLR}             & 71.74              &  8.10           & 56.92            &  \multicolumn{1}{c|}{42.59}            \\  
%     \multicolumn{1}{|c|}{Barlow Twins}      & 42.00              &  7.53           & 64.82            &  \multicolumn{1}{c|}{49.43}            \\  
%     \multicolumn{1}{|c|}{VICReg}            & 36.04              &  4.95           & 56.92            &  \multicolumn{1}{c|}{50.26}            \\ \hline
%     \multicolumn{1}{|c|}{\oursimclr (ours)} & 73.81              &  18.15          & 86.98            &  \multicolumn{1}{c|}{57.62}            \\                   
%     \multicolumn{1}{|c|}{\ourbyol (ours)}   & \FB{74.04}         &  15.96          & \FB{87.56}       &  \multicolumn{1}{c|}{\FB{59.15}}        \\  
%     \multicolumn{1}{|c|}{\ourbarlow (ours)} & 74.24              &  16.26          & 85.08            &  \multicolumn{1}{c|}{58.55}            \\                   
%     \multicolumn{1}{|c|}{\ourvicreg (ours)} & 72.60              &  \FB{19.26}     & 85.36            &  \multicolumn{1}{c|}{57.06}            \\ \hline
% \end{tabular}
% }
% \end{center}
% \label{tab:all-datasets-metrics-sa}
% \label{tab:all-datasets-metrics-ma}
% \end{table*}


% % \begin{table*}[ht!]
% % \caption{Classification accuracy of \ourmethod and baseline SSL method on four datasets, each in \strongaug and \weakaug setting. The set of DA used for \strongaug are \texttt{random-resized-crop}, \texttt{random-horizontal-flip}, \texttt{color-jitter}, \texttt{gray-scale}, \texttt{gaussian-blur} and \texttt{solarization} and for \weakaug the only DA used is \texttt{random horizontal flip}. We mark the best performing score in \textbf{bold}.}
% % \begin{center}
% %  \resizebox{\linewidth}{!}{%
% % \begin{tabular}{cllllllllllll}
% %     \hline
% %     \multicolumn{1}{|c}{}           & \multicolumn{1}{c}{\cifarten}            & \multicolumn{1}{c}{\aircrafts}         & \multicolumn{1}{c}{\pathmnist} &      \multicolumn{1}{c|}{\tissuemnist}            \\
% %     \hline
% %     \hline
% %     \multicolumn{1}{|c|}{SimCLR}            &  \multicolumn{1}{l|}{88.26}     &  \multicolumn{1}{l|}{39.27} & \multicolumn{1}{l|}{ 91.56        }    &             
% %     \multicolumn{1}{|c|}{BYOL}              &  \multicolumn{1}{l|}{-----}     &  \multicolumn{1}{l|}{-----} & \multicolumn{1}{l|}{ 91.24        }    &             
% %     \multicolumn{1}{|c|}{NNCLR}             &  \multicolumn{1}{l|}{-----}     &  \multicolumn{1}{l|}{-----} & \multicolumn{1}{l|}{ -----        }    &    
% %     \multicolumn{1}{|c|}{Barlow Twins}      &  \multicolumn{1}{l|}{88.89}     &  \multicolumn{1}{l|}{-----} & \multicolumn{1}{l|}{ 92.23        }    &    
% %     \multicolumn{1}{|c|}{VICReg}            &  \multicolumn{1}{l|}{89.34}     &  \multicolumn{1}{l|}{33.21} & \multicolumn{1}{l|}{ 92.27        }    &                                                                                                                    
% %     \multicolumn{1}{|c|}{\oursimclr (ours)} &  \multicolumn{1}{l|}{89.57}     &  \multicolumn{1}{l|}{49.57} & \multicolumn{1}{l|}{\textbf{92.19}}    &                     
% %     \multicolumn{1}{|c|}{\ourbyol (ours)}   &  \multicolumn{1}{l|}{-----}     &  \multicolumn{1}{l|}{45.48} & \multicolumn{1}{l|}{91.05         }    &    
% %     \multicolumn{1}{|c|}{\ourbarlow (ours)} &  \multicolumn{1}{l|}{88.39}     &  \multicolumn{1}{l|}{-----} & \multicolumn{1}{l|}{91.55         }    &                     
% %     \multicolumn{1}{|c|}{\ourvicreg (ours)} &  \multicolumn{1}{l|}{89.68}     &  \multicolumn{1}{l|}{-----} & \multicolumn{1}{l|}{91.88         }    &                     

    
% %     \hline
% % \end{tabular}
% % }
% % \end{center}
% % \label{tab:all-datasets-metrics}
% % \end{table*}


==> tabs/strong_aug_results.tex <==
\begin{table*}[ht!]
\caption{Classification accuracy of \ourmethod and baseline SSL method on four datasets, each in \strongaug and \weakaug setting. The set of DA used for \strongaug are \texttt{random-resized-crop}, \texttt{random-horizontal-flip}, \texttt{color-jitter}, \texttt{gray-scale}, \texttt{gaussian-blur} and \texttt{solarization} and for \weakaug the only DA used is \texttt{random horizontal flip}. We mark the best performing score in \textbf{bold}.}
\begin{center}
 \resizebox{\linewidth}{!}{%
\begin{tabular}{clllllllllllllllll}
    \hline
    \multicolumn{1}{|c}{}    & \multicolumn{2}{c}{\rotatebox[origin=c]{90}{\cifarten}}            & \multicolumn{2}{c}{\rotatebox[origin=c]{90}{\cifarhundred}}         & \multicolumn{2}{c}{\rotatebox[origin=c]{90}{\svhn}} &      \multicolumn{2}{c|}{\rotatebox[origin=c]{90}{\aircrafts}}            \\
    \hline
    \multicolumn{1}{|c|}{Methods}  &  \strongaug & \multicolumn{1}{c|}{K}  &  \strongaug & \multicolumn{1}{c|}{K}  &  \strongaug & \multicolumn{1}{c|}{K} &  \strongaug & \multicolumn{1}{c|}{K}  \\
    
    \hline
    \hline
    \multicolumn{1}{|c|}{SimCLR}  &   87.57 &  \multicolumn{1}{l|}{1} &         61.57 &  \multicolumn{1}{l|}{1} &      7.70 &  \multicolumn{1}{l|}{1}     &  37.88 &  \multicolumn{1}{l|}{1}      \\           
    \multicolumn{1}{|c|}{BYOL}                &  86.97 &  \multicolumn{1}{l|}{1}         &  59.48 &  \multicolumn{1}{l|}{1} &         43.97 &  \multicolumn{1}{l|}{1} &  87.04 &  \multicolumn{1}{l|}{1}                 \\           
    \multicolumn{1}{|c|}{NNCLR}        &  86.06 &  \multicolumn{1}{l|}{1}    &    62.46 &  \multicolumn{1}{l|}{1} &         20.08 &  \multicolumn{1}{l|}{1} &  90.85 &  \multicolumn{1}{l|}{1}        \\  

    \multicolumn{1}{|c|}{Barlow Twins}      &  86.45 &  \multicolumn{1}{l|}{1}    &  - &  \multicolumn{1}{l|}{1} &         35.91 &  \multicolumn{1}{l|}{1} &  91.71 &  \multicolumn{1}{l|}{1}         \\  
    
    \multicolumn{1}{|c|}{VICReg}                         &  \textbf{89.92} &  \multicolumn{1}{l|}{1}     &    -      &  \multicolumn{1}{l|}{1} &   26.29 &  \multicolumn{1}{l|}{1}  \\           
    \hline
    \multicolumn{1}{|c|}{\oursimclr (ours)}                 &  85.53 &  \multicolumn{1}{l|}{2}            &  59.21 &  \multicolumn{1}{l|}{1} &            \textbf{61.05} &  \multicolumn{1}{l|}{5} &  83.80 &  \multicolumn{1}{l|}{2}                \\                   
    
    \multicolumn{1}{|c|}{\ourbyol (ours)}                 &  83.51 &  \multicolumn{1}{l|}{2}              &  56.33 &  \multicolumn{1}{l|}{1} &            64.47 &  \multicolumn{1}{l|}{2} &  66.41 &  \multicolumn{1}{l|}{2}  \\  
    
    \multicolumn{1}{|c|}{\ourbarlow (ours)}               &  81.93 &  \multicolumn{1}{l|}{2}              & - & \multicolumn{1}{l|}{1} &            \textbf{60.79} &  \multicolumn{1}{l|}{2} &  80.19 &  \multicolumn{1}{l|}{2}  \\                   

    \multicolumn{1}{|c|}{\ourvicreg (ours)}               &  85.54 &  \multicolumn{1}{l|}{2}              &  - &  \multicolumn{1}{l|}{1} &  57.48 &  \multicolumn{1}{l|}{5}                 &  87.00 &  \multicolumn{1}{l|}{2}                   \\                   

    
    \hline
\end{tabular}
}
\end{center}
\label{tab:all-datasets-metrics}
\end{table*}

